Fully dynamic data structure for LCE queries in compressed space

A Longest Common Extension (LCE) query on a text $T$ of length $N$ asks for the length of the longest common prefix of suffixes starting at given two positions. We show that the signature encoding $\mathcal{G}$ of size $w = O(\min(z \log N \log^* M, N))$ [Mehlhorn et al., Algorithmica 17(2):183-198, 1997] of $T$, which can be seen as a compressed representation of $T$, has a capability to support LCE queries in $O(\log N + \log \ell \log^* M)$ time, where $\ell$ is the answer to the query, $z$ is the size of the Lempel-Ziv77 (LZ77) factorization of $T$, and $M \geq 4N$ is an integer that can be handled in constant time under word RAM model. In compressed space, this is the fastest deterministic LCE data structure in many cases. Moreover, $\mathcal{G}$ can be enhanced to support efficient update operations: After processing $\mathcal{G}$ in $O(w f_{\mathcal{A}})$ time, we can insert/delete any (sub)string of length $y$ into/from an arbitrary position of $T$ in $O((y+ \log N\log^* M) f_{\mathcal{A}})$ time, where $f_{\mathcal{A}} = O(\min \{ \frac{\log\log M \log\log w}{\log\log\log M}, \sqrt{\frac{\log w}{\log\log w}} \})$. This yields the first fully dynamic LCE data structure. We also present efficient construction algorithms from various types of inputs: We can construct $\mathcal{G}$ in $O(N f_{\mathcal{A}})$ time from uncompressed string $T$; in $O(n \log\log n \log N \log^* M)$ time from grammar-compressed string $T$ represented by a straight-line program of size $n$; and in $O(z f_{\mathcal{A}} \log N \log^* M)$ time from LZ77-compressed string $T$ with $z$ factors. On top of the above contributions, we show several applications of our data structures which improve previous best known results on grammar-compressed string processing.

==> static_index.tex <==
\section{Dynamic Compressed Index}\label{sec:static_section}

In this section, we present our dynamic compressed index based on signature encoding.
As already mentioned in Section~\ref{sec:related_work}, 
our strategy for pattern matching is different from that of Alstrup et al.~\cite{LongAlstrup}.
It is rather similar to the one taken in the static index for SLPs of Claude and Navarro~\cite{claudear:_self_index_gramm_based_compr}.
Besides applying their idea to run-length ACFGs, we show how to speed up pattern matching by utilizing the properties of signature encodings.
%although it use the signature encoding
%our searching algorithm is based on the property of context free grammar which generates a single text, 
%which is the fact that any pattern of at least length 2 occurs between at least two variables if the pattern occurs in $T$. 

The rest of this section is organized as follows:
In Section~\ref{sec:SLPIndex}, we briefly review the idea for the SLP index of Claude and Navarro~\cite{claudear:_self_index_gramm_based_compr}.
In Section~\ref{subsec:RunLen}, we extend their idea to run-length ACFGs.
In Section~\ref{subsec:StaticIndexSigDic}, we consider an index on signature encodings and
improve the running time of pattern matching by using the properties of signature encodings.
In Section~\ref{subsec:DynIndexSigEnc}, we show how to dynamize our index.

\subsection{Static Index for SLP}\label{sec:SLPIndex}
We review how the index in~\cite{claudear:_self_index_gramm_based_compr}
for SLP $\mathcal{S}$ generating a string $T$ computes $\Occ(P,T)$ for a given string $P$.
The key observation is that, any occurrence of $P$ in $T$
can be uniquely associated with the lowest node that covers the occurrence of $P$ in the derivation tree.
As the derivation tree is binary, if $|P| > 1$, then the node is labeled with some variable $X \in \mathcal{V}$ such that
$P_1$ is a suffix of $X.{\rm left}$ and $P_2$ is a prefix of $X.{\rm right}$, where $P = P_1P_2$ with $1 \leq |P_1| < |P|$.
Here we call the pair $(X, |X.{\rm left}| - |P_1| + 1)$ a \emph{primary occurrence} of $P$.
Then, we can compute $\Occ(P, T)$ by first computing such a primary occurrence and
enumerating the occurrences of $X$ in the derivation tree.

Formally, we define the \emph{primary occurrences} of $P$ as follows.
\begin{definition}[The set of primary occurrences of $P$]\label{def:primary}
For a string $P$ with $|P| > 1$ and an integer $1 \leq j < |P|$, 
we define $\mathit{pOcc}_{\mathcal{S}}(P, j)$ and $\mathit{pOcc}_{\mathcal{S}}(P)$ as follows:
\begin{eqnarray*}
 \mathit{pOcc}_{\mathcal{S}}(P, j) & = & \{ (X, |X.{\rm left}| - j + 1) \mid X \in \mathcal{V},\\
                                   && \text{$P[..j]$ is a suffix of $X.{\rm left}$, $P[j+1..]$ is a prefix of $X.{\rm right}$}\},\\
 \mathit{pOcc}_{\mathcal{S}}(P) & = & \bigcup_{1 \leq j < |P|} \mathit{pOcc}_{\mathcal{S}}(P, j),\\
\end{eqnarray*}
We call each element of $\mathit{pOcc}_{\mathcal{S}}(P)$ a primary occurrence of $P$.
\end{definition}
%We can compute an occurrence position of $P$ in $T$ by an occurrence position of $P$ in $\val{X_i}$ 
%and an occurrence position of $X_i$ in $\mathcal{S}$ for some variable $X_i$. 
The set $\mathit{Occ}(P,T)$ of occurrences of $P$ in $T$ is represented by $\mathit{pOcc}_{\mathcal{S}}(P)$ as follows.
\begin{observation}\label{ob:OccurrenceSLP}
For any string $P$,
\begin{eqnarray*}
 \mathit{Occ}(P,T) &=&
  \begin{cases}
  \{ j+k-1 \mid (X, j) \in \mathit{pOcc}_{\mathcal{S}}(P), k \in \mathit{vOcc}(X, S)\} & \mbox{ if } |P| > 1,\\
  \mathit{vOcc}(X ,S) ((X \rightarrow P) \in \mathcal{D}) & \mbox{ if } |P| = 1.\\
  \end{cases}\\
\end{eqnarray*}
\end{observation}
%Observation~\ref{ob:OccurrenceSLP} means that 
%there exists a primary occurrence $(X_i,d)$ of $P$ such that 
%$X_i$ occurs at position $c-d$ in $S$ for $c \in \Occ(P,T)$. 

By Observation~\ref{ob:OccurrenceSLP},
the task is to compute $\mathit{pOcc}_{\mathcal{S}}(P)$ and $\mathit{vOcc}(X,S)$ efficiently.
Note that $\mathit{vOcc}(X,S)$ can be computed in $O(|\mathit{vOcc}(X,S)| h)$ time
by traversing the DAG in a reversed direction (i.e., using $\mathit{parents}(X)$ function recursively) from $X$ to the source,
where $h$ is the height of the derivation tree of $S$.
Hence, in what follows, we focus on how to compute $\mathit{pOcc}_{\mathcal{S}}(P)$ for a string $P$ with $|P| > 1$.
In order to compute $\mathit{pOcc}_{\mathcal{S}}(P,j)$,
we use a data structure to solve the following problem:
\begin{problem}[Two-Dimensional Orthogonal Range Reporting Problem]\label{problem:2D}
Let $\mathcal{X}$ and $\mathcal{Y}$ denote subsets of two ordered sets,
and let $\mathcal{R} \subseteq \mathcal{X} \times \mathcal{Y}$ be a set of points on the two-dimensional plane,
where $|\mathcal{X}|, |\mathcal{Y}| \in O(|\mathcal{R}|)$.
A data structure for this problem supports a query $\mathit{report}_{\mathcal{R}}(x_1,x_2,y_1,y_2)$;
given a rectangle $(x_1,x_2,y_1,y_2)$ with $x_1, x_2 \in \mathcal{X}$ and $y_1, y_2 \in \mathcal{Y}$, 
returns $\{ (x,y) \in \mathcal{R} \mid x_1 \leq x \leq x_2, y_1 \leq y \leq y_2 \}$.
% Let $\mathcal{R}$ be a set of points on a two-dimensional plane, where
% $\mathcal{X} = \{ x \mid (x, y) \in \mathcal{R} \}$ and $\mathcal{Y} = \{ y \mid (x, y) \in \mathcal{R} \}$) are ordered sets.
% The problem is to construct a data structure to support a query $\mathit{report}_{\mathcal{R}}(x_1,x_2,y_1,y_2)$;
% given a rectangle $(x_1,x_2,y_1,y_2)$, return $\{ (x,y) \in \mathcal{R} \mid x_1 \leq x \leq x_2, y_1 \leq y \leq y_2 \}$.
\end{problem}

Data structures for Problem~\ref{problem:2D} are widely studied in computational geometry.
% We can use any of such data structures working in $O(|\mathcal{R}|)$ space.
There is even a dynamic variant, which we finally use for our dynamic index in Section~\ref{subsec:DynIndexSigEnc}.
% Until then, we describe time complexities in an abstracted manner:
% We use any static data structure that occupies $O(|\mathcal{R}|)$ space and
% supports range reporting queries in $O(\hat{q}_{|\mathcal{R}|} + q_{|\mathcal{R}|} \mathit{qocc})$ time,
% where $\mathit{qocc}$ is the number of points to report.
Until then, we just use any static data structure that occupies $O(|\mathcal{R}|)$ space and
supports queries in $O(\hat{q}_{|\mathcal{R}|} + q_{|\mathcal{R}|} \mathit{qocc})$ time with $\hat{q}_{|\mathcal{R}|} = O(\log |\mathcal{R}|)$,
where $\mathit{qocc}$ is the number of points to report.

Now, given an SLP $\mathcal{S}$, we consider a two-dimensional plane defined by 
$\mathcal{X} = \{ X.{\rm left}^{R} \mid X \in \mathcal{V} \}$ and $\mathcal{Y}  = \{ X.{\rm right} \mid X \in \mathcal{V} \}$,
where elements in $\mathcal{X}$ and $\mathcal{Y}$ are sorted by lexicographic order.
Then consider a set of points $\mathcal{R} = \{ (X.{\rm left}^{R}, X.{\rm right}) \mid X \in \mathcal{V} \}$.
For a string $P$ and an integer $1 \leq j < |P|$,
let $y_1^{(P,j)}$ (resp. $y_2^{(P,j)}$) denote the lexicographically smallest (resp. largest) element 
in $\mathcal{Y}$ that has $P[j+1..]$ as a prefix.
If there is no such element, it just returns NIL and we can immediately know that $\mathit{pOcc}_{\mathcal{S}}(P,j) = \emptyset$.
% Note that $y_1^{(P,j)}$ and $y_2^{(P,j)}$ can be computed in $O(|P| \log n)$ time by binary search on $^mathcal{Y}$.
We also define $x_1^{(P,j)}$ and $x_2^{(P,j)}$ in a similar way over $\mathcal{X}$, i.e.,
$x_1^{(P,j)}$ (resp. $x_2^{(P,j)}$) is the lexicographically smallest (resp. largest) element in $\mathcal{X}$ that has $P[..j]^{R}$ as a prefix.
Then, $\mathit{pOcc}_{\mathcal{S}}(P, j)$ can be computed by a query $\mathit{report}_{\mathcal{R}}(x_1^{(P,j)}, x_2^{(P,j)}, y_1^{(P,j)}, y_2^{(P,j)})$.
See also Example~\ref{ex:SLPGrid}.
\begin{example}[SLP]\label{ex:SLPGrid}
Let $\mathcal{S}$ be the SLP of Example~\ref{ex:SLP}. 
Then, 
\begin{eqnarray*}
\mathcal{X} &=& \{ x_1, x_4, x_2, x_8, x_5, x_9, x_6, x_{10}, x_{11}, x_3, x_7 \}, \\
\mathcal{Y} &=& \{ y_1, y_8, y_2, y_7, y_9, y_3, y_4, y_{5}, y_{6}, y_{10}, y_{11} \}, \\
\end{eqnarray*}
where 
$x_i = \val{X_i}^{R}$, $y_i = \val{X_i}$ for any $X_i \in \mathcal{V}$.
% and $p_i = (X_i.{\rm left}^{R}, X_i.{\rm right})$ for any $X_i \in \mathcal{V}$ with $X_i \rightarrow X_l X_r$.
Given a pattern $P = BCAB$, then 
$\mathit{pOcc}_{\mathcal{S}}(P,1) = \{ (X_{6},3), (X_{11}, 10 )\}$, 
$\mathit{pOcc}_{\mathcal{S}}(P,2) = \{ (X_{9},1) \}$, 
$\mathit{pOcc}_{\mathcal{S}}(P,3) = \phi$, 
$\mathit{vOcc}_{\mathcal{S}}(X_{6},S) = \{1,11\}$, 
$\mathit{vOcc}_{\mathcal{S}}(X_{9},S) = \{7\}$ and 
$\mathit{vOcc}_{\mathcal{S}}(X_{11},S) = \{1\}$. 
Hence $\mathit{pOcc}_{\mathcal{S}}(P) = \{ (X_{6},3), (X_{11}, 10), (X_{9},1)\}$ and 
$\mathit{Occ}(P,T) = \{3,7,10,13\}$. 
See also Fig.~\ref{fig:grid}. 
\end{example}
\begin{figure}[ht]
\begin{center}
  \includegraphics[scale=0.48]{figure/grid.eps}
  \caption{
  The grid represents the relation between $\mathcal{X}$, $\mathcal{Y}$ and $\mathcal{R}$ of Example~\ref{ex:SLPGrid}. 
  The red rectangle is a query rectangle $(x^{(P,1)}_1,x^{(P,1)}_2,y^{(P,1)}_1,y^{(P,1)}_2)$, where 
  $x^{(P,1)}_1 = x_2$, $x^{(P,1)}_2 = x_{11}$, $y^{(P,1)}_1 = y_5$ and $y^{(P,1)}_2 = y_{11}$. 
  Therefore, $\mathit{report}_{\mathcal{R}}(x^{(P,1)}_1,x^{(P,1)}_2,y^{(P,1)}_1,y^{(P,1)}_2) = \{ X_{6}, X_{11} \}$.
  }
  \label{fig:grid}
\end{center}
\end{figure}

We can get the following result:
\begin{lemma}\label{lem:LinearSpaceIndexOfSLP}
% For an SLP $\mathcal{S}$ of size $n$ generating string $T$,
% there exists an index for $\mathcal{S}$ of size $O(n)$, which computes 
% $\mathit{Occ}(P,T)$ in $O(m ((h + m) \log n + \hat{q}_{\mathcal{R}}) + (h + q_{\mathcal{R}}) |\mathit{Occ}(P,T)|)$ time for any pattern $P$.
For an SLP $\mathcal{S}$ of size $n$,
there exists a data structure of size $O(n)$ that computes, given a string $P$,
$\mathit{pOcc}_{\mathcal{S}}(P)$ in $O(|P| (h + |P|) \log n + q_{n} |\mathit{pOcc}_{\mathcal{S}}(P)|)$ time.
\end{lemma}
\begin{proof}
For every $1 \leq j < |P|$, we compute $\mathit{pOcc}_{\mathcal{S}}(P, j)$ by 
$\mathit{report}_{\mathcal{R}}(x_1^{(P,j)}, x_2^{(P,j)}, y_1^{(P,j)}, y_2^{(P,j)})$.
We can compute $y_1^{(P,j)}$ and $y_2^{(P,j)}$ in $O((h + |P|) \log n)$ time by binary search on $\mathcal{Y}$,
where each comparison takes $O(h + |P|)$ time for expanding the first $O(|P|)$ characters of variables subjected to comparison.
In a similar way, $x_1^{(P,j)}$ and $x_2^{(P,j)}$ can be computed in $O((h + |P|) \log n)$ time.
Thus, the total time complexity is 
$O(|P| ((h + |P|) \log n + \hat{q}_{n}) + q_{n} |\mathit{pOcc}_{\mathcal{S}}(P)|) = O(|P| (h + |P|) \log n + q_{n} |\mathit{pOcc}_{\mathcal{S}}(P)|)$.
% Finally, $\mathit{pOcc}_{\mathcal{S}}(P)$ can be computed in the query reports primary occurrences in $O(q_{n})$ time each,
% after spending $O(\hat{q}_{n})$ time for the warming-up cost.
\qed
\end{proof}

% Now, let $\Lambda_{\mathcal{S}}$ denote a data structure of Lemma~\ref{lem:RangeQuery} for such $\mathcal{R}$. 
% Note that we can represent $\mathcal{X}, \mathcal{Y}$ and $\mathcal{R}$ in $O(n)$ space for an SLP $\mathcal{S}$
% because we do not need store explicit values of $X_{i}.{\rm left}^{R}$ and $X_{i}.{\rm right}$ for $X_{i} \in \mathcal{V}$.
% Then we get the following fact.
% \begin{fact}\label{fact:LinearSpaceIndexOfSLP}
% There exists a data structure for an SLP $\mathcal{S}$ of size $n$, which computes
% $\mathit{pOcc}_{\mathcal{S}}(P,j)$ for given $x_1^{(P,j)}, x_2^{(P,j)}, y_1^{(P,j)}$ and $y_2^{(P,j)}$ 
% in $O(\log n + \mathit{occ} (\log n/ \log \log n))$ time, occupying $O(n)$ space, 
% where $P$ is a string and $j$ is an integer.
% \end{fact}
 
\subsection{Static Index for Run-length ACFG}\label{subsec:RunLen}
In this subsection, we extend the idea for the SLP index described in Section~\ref{sec:SLPIndex} to run-length ACFGs.
Consider occurrences of string $P$ with $|P| > 1$ in run-length ACFG $\mathcal{G} = (\Sigma, \mathcal{V}, \mathcal{D}, S)$ generating string $T$.
The difference from SLPs is that we have to deal with occurrences of $P$
that are covered by a node labeled with $e \rightarrow \hat{e}^{d}$ but not covered by any single child of the node in the derivation tree.
In such a case, there must exist $P = P_1P_2$ with $1 \leq |P_1| < |P|$ such that
$P_1$ is a suffix of $e.{\rm left} = \valp{\hat{e}}$ and $P_2$ is a prefix of $e.{\rm right} = \valp{\hat{e}^{d-1}}$.
Let $j = |\val{\hat{e}}| - |P_1| + 1$ be a position in $\valp{\hat{e}^{d}}$ where $P$ occurs,
then $P$ also occurs at $j + c |\val{\hat{e}}|$ in $\valp{\hat{e}^{d}}$ for every positive integer
$c$ with $j + c |\val{\hat{e}}| + |P| - 1 \leq |\valp{\hat{e}^{d}}|$.
Remarking that we apply Definition~\ref{def:primary} of primary occurrences to run-length ACFGs as they are,
we formalize our observation to compute $\mathit{Occ}(P,T)$ as follows:
\begin{observation}
For any string $P$ with $|P| > 1$,
$\mathit{Occ}(P,T) = \{ j+k+c-1 \mid (e, i) \in \mathit{pOcc}_{\mathcal{G}}(P), 
c \in \{ 0 \} \cup \mathit{Run}_{\mathcal{G}}(e,j,|P|), k \in \mathit{vOcc}(e,S)\}$, where 
\begin{eqnarray*}
  \mathit{Run}_{\mathcal{G}}(e, j, |P|) & = & 
   \begin{cases}
    \{ c |\val{\hat{e}}| \mid 1 \leq c, j + c |\val{\hat{e}}| + |P| - 1 \leq |\valp{\hat{e}^{d}}| \} & \mbox{if } e \rightarrow \hat{e}^d, \\
	\emptyset & \mbox{otherwise.} \\
   \end{cases}
\end{eqnarray*}
\end{observation}
% By the above observation, we can construct an index for a run-length ACFG in the same way as for SLPs.
By the above observation, we can get the same result for a run-length ACFG as for an SLP in Lemma~\ref{lem:LinearSpaceIndexOfSLP}.

% \tnnote*{the difference point}{
% Each occurrence of $P$ of at least length $2$ is divided by $e_{\ell}$ and $e_{r}$ 
% in a variable $e \rightarrow e_{\ell}e_{r} \in \mathcal{D}$, 
% or is divided in a variable $e \rightarrow \hat{e}^k \in \mathcal{D}$. 
% The 'divide' in $e \rightarrow \hat{e}^k \in \mathcal{D}$ means that 
% there exist $P = P_1P_2$ and an integer $1 \leq j < k$ such that 
% $P_1$ is a suffix of $\valp{\hat{e}^{j}}$ and $P_2$ is a prefix of $\valp{\hat{e}^{k-j}}$. 
% Since $\val{e}$ is the run of $\hat{e}$, if such integer $j > 1$ exists then $j = 1$ also exists.
% }
% \begin{observation}\label{ob:RunPrimaryOccurrence}
% For any string $P$, integer $1 \leq j < |P|$ and variable $e \rightarrow \hat{e}^{d} \in \mathcal{D}$, 
% $P[..j]$ is a suffix of $\val{\hat{e}}$ and $P[j+1..]$ is a prefix of $\val{\hat{e}}^{d-1}$ if and only if 
% $P[..j]$ is a suffix of $\val{\hat{e}}^{q}$ and $P[j+1..]$ is a prefix of $\val{\hat{e}}^{d-q}$ for $1 < q < x$, 
% where $x$ is the maximum integer such that $|P[j+1..]| \leq |\val{\hat{e}}^{d-x}|$.
% \end{observation}
% Observation~\ref{ob:RunPrimaryOccurrence} means that 
% we can compute every occurrence of $P$ of at least length $2$, 
% which is divided in a variable $e \rightarrow \hat{e}^k \in \mathcal{D}$, 
% by the occurrences which is divided by $e.{\rm left}$ and $e.{\rm right}$. 
% Hence we define Definition~\ref{def:primary} of the run-length ACFG version.
% The definition is the same as the one of the SLP version.
% Then Observation~\ref{ob:RunPrimaryOccurrence} implies the following observation holds. 
% This is the run-length ACFGs version of Observation~\ref{ob:OccurrenceSLP}.
% \begin{observation}
% For any string $P$ with $|P| > 1$, then 
% $\mathit{Occ}(P,T) = \{ i+k+c-1 \mid (e, i) \in \mathit{pOcc}_{\mathcal{G}}(P), 
% c \in \{ 0 \} \cup \mathit{Run}_{\mathcal{G}}(e,i,|P|), k \in \mathit{vOcc}(e,S)\}$ 
% holds, where 
% \begin{eqnarray*}
%   \mathit{Run}_{\mathcal{G}}(e, i, k) & = & 
%    \begin{cases}
%     \{ |\val{\hat{e}}^1|, \ldots, |\val{\hat{e}}^x| \} & \mbox{if } e \rightarrow \hat{e}^k \\
% 	\phi & \mbox{otherwise } \\
%    \end{cases}
% \end{eqnarray*}
% and $x$ is the value in Observation~\ref{ob:RunPrimaryOccurrence}. 
% \end{observation}

\subsection{Static Index for Signature Encoding}\label{subsec:StaticIndexSigDic}
We can apply the result of Section~\ref{subsec:RunLen} to signature encodings 
because signature encodings are run-length ACFGs, i.e.,
we can compute $\mathit{Occ}(P,T)$ by querying
$\mathit{report}_{\mathcal{R}}(x_1^{(P,j)}, x_2^{(P,j)},y_1^{(P,j)}, y_2^{(P,j)})$
for ``every'' $1 \leq j < |P|$.
However, the properties of signature encodings allow us to speed up pattern matching
as summarized in the following two ideas:
(1) We can efficiently compute $x_1^{(P,j)}, x_2^{(P,j)}, y_1^{(P,j)}$ and $y_2^{(P,j)}$
using LCE queries in compressed space (Lemma~\ref{lem:ComputePatternRange}).
(2) We can reduce the number of $\mathit{report}_{\mathcal{R}}$ queries from 
$O(|P|)$ to $O(\log |P| \log^* M)$ by using the property of the common sequence of $P$ (Lemma~\ref{lem:pattern_occurrence_lemma1}).
%Recall that Fact~\ref{fact:LinearSpaceIndexOfSLP} implies 
%that we need $|P|$ times range reporting to compute $\Occ(P,T)$. 

% For (1), we show the following lemma.
\begin{lemma}\label{lem:ComputePatternRange}
Assume that we have the DAG for a signature encoding $\mathcal{G} = (\Sigma, \mathcal{V}, \mathcal{D}, S)$ 
of size $w$ and $\mathcal{X}$ and $\mathcal{Y}$ of $\mathcal{G}$.
Given a signature $\id{P} \in \mathcal{V}$ for a string $P$ and an integer $j$, 
we can compute $x_1^{(P,j)}, x_2^{(P,j)}, y_1^{(P,j)}$ and $y_2^{(P,j)}$ in $O(\log w (\log N + \log |P| \log^* M))$ time.
\end{lemma}
\begin{proof}
By Lemma~\ref{lem:sub_operation_lemma} and Fact~\ref{obs:RandomAccess},
we can compute $x_1^{(P,j)}$ and $x_2^{(P,j)}$ 
on $\mathcal{X}$ by binary search in $O(\log w (\log N + \log |P| \log^* M))$ time.
Similarly, we can compute $y_1^{(P,j)}$ and $y_2^{(P,j)}$ in the same time. 
\qed
\end{proof}

% For (2), we show the following lemma.
\begin{lemma}\label{lem:pattern_occurrence_lemma1}
  Let $P$ be a string with $|P| > 1$.
  If $|\pow{0}{P}| = 1$, then $\mathit{pOcc}_{\mathcal{G}}(P) = \mathit{pOcc}_{\mathcal{G}}(P, 1)$.
  If $|\pow{0}{P}| > 1$, then $\mathit{pOcc}_{\mathcal{G}}(P) = \bigcup_{j \in \mathcal{P}} \mathit{pOcc}_{\mathcal{G}}(P, j)$, where
  $u$ is the common sequence of $P$ and $\mathcal{P} = \{ |\valp{u[1..i]}| \mid 1 \leq i < |u|, u[i] \neq u[i+1] \}$.
\end{lemma}
\begin{proof}
If $|\pow{0}{P}| = 1$, then $P = a^{|P|}$ for some character $a \in \Sigma$.
In this case, $P$ must be contained in a node labeled with a signature 
$e \rightarrow \hat{e}^{d}$ such that $\hat{e} \rightarrow a$ and $d \geq |P|$.
Hence, all primary occurrences of $P$ can be found by $\mathit{pOcc}_{\mathcal{G}}(P, 1)$.

If $|\pow{0}{P}| > 1$, we consider the common sequence $u$ of $P$.
Recall that $u$ occurs at position $j$ in $e$ for any $(e,j) \in \mathit{pOcc}(P)$ by Lemma~\ref{lem:common_sequence2}. 
Hence at least $\mathit{pOcc}_{\mathcal{G}}(P) = \bigcup_{i \in \mathcal{P'}} \mathit{pOcc}_{\mathcal{G}}(P,i)$ holds, 
where $\mathcal{P'} = \{|\valp{u[1]}|, \ldots, |\valp{u[..|u|-1]}|\}$.
Moreover, we show that $\mathit{pOcc}_{\mathcal{G}}(P,i) = \emptyset$ for any $i \in \mathcal{P'}$ with $u[i] = u[i+1]$.
Note that $u[i]$ and $u[i+1]$ are encoded into the same signature in the derivation tree of $e$, and
that the parent of two nodes corresponding to $u[i]$ and $u[i+1]$ has a signature $e'$ in the form $e' \rightarrow u[i]^{d}$.
Now assume for the sake of contradiction that $e = e'$.
By the definition of the primary occurrences, $i = 1$ must hold, and hence, $\shrink{0}{P}[1] = u[1] \in \Sigma$.
This means that $P = u[1]^{|P|}$, which contradicts $|\pow{0}{P}| > 1$.
Therefore the statement holds.
\qed
%Consider a common sequence of $P$ of Lemma~\ref{lem:common_sequence2}
%and see also Fig.~\ref{fig:CommonSequence}.
%Assume that there exists an integer $i$ and a signature $e \in \mathcal{V}$ such that 
%$\mathit{pOcc}_{\mathcal{G}}(e,P,i) = 1$ 
%and $i \not \in \mathcal{P'}$. 
%We consider two cases on $i$: 
%Case (1) There exists an integer $c$ which satisfies $|\valp{u[..c-1]}| < i < |\valp{u[..c]}|$. 
%Case (2) There exist an integer $d,r$ such that $i = |\valp{v_1 \cdots v_{d-1}}| + |\valp{q^r}|$, 
%$1 \leq d \leq k$ and $1 \leq r < r_d$ where $q_{j}^{r_j} = v_j$ for $1 \leq j \leq k$.
%(1) Let $j = |e.{\rm left}| - i + 1$.  
%Then $\vOcc(u[c],e, j + |\val{u_1 \cdots u_{c-1}}|) = 0$ holds clearly. 
%This contradicts with Lemma~\ref{lem:common_sequence2}. 
%(2) Consider two sub-cases: (i) $e \rightarrow e_le_r (e_l \not = e_r)$ (ii) $e \rightarrow q^{m}$. 
%Note that $e_l \not = e_r$ hold for $e \rightarrow e_{\ell}e_{r} \in \mathcal{D}$ by the definition of the signature encoding. 
%(i) $|\val{e_l}| - |\val{q_d}| + 1 \in \mathit{vOcc}(q_d,e_l)$ and 
%$1 \in \mathit{vOcc}(q_d,e_r)$ hold. In other word, $v_d$ 
%(or a maximal run which contains $v_d$) is not encoded to a single signature 
%in the signature encoding of $T$. This contradicts the definition of signature encoding. 
%(ii) Similarly, $|\val{q}| - |\val{q_d}| + 1 \in \mathit{vOcc}(q_d,q)$ and 
%$1 \in \mathit{vOcc}(q_d,q)$ hold. If $q_d \not = q$, 
%this is the same as Case (i). Otherwise, $q_d = q$. 
%By the definition of $\mathit{pOcc}(e,P)$, 
%$e.{\rm left} = \val{q} = \valp{v_1 \cdots v_{d-1} \cdot q_d^r}$. 
%This holds when $r = 1$ and $d = 1$, 
%then $q = q_d \rightarrow a \in \Sigma$. 
%Next, $\valp{q_d^{r_d-r} \cdot v_{d+1} \cdots v_k}$ is a prefix of $e.{\rm right} = a^{m-1}$. 
%Since $q_{d} \not = q_{d+1}$ and $k > d$ ($d = 1$ and $k > 1$), 
%$\valp{q_d^{r_d-r} \cdot v_{d+1} \cdots v_k}$ is not a prefix of $e.{\rm right}$.
%Therefore, Lemma \ref{lem:pattern_occurrence_lemma1} holds. 
%\qed
\end{proof}

% Note that we use $\mathcal{H}(f_{\mathcal{A}}, f'_{\mathcal{A}})$ that represents the signature encoding of $\mathcal{G}$,
% but do not modify it as the common sequence of $P$ is constructed temporally and deleted soon after pattern matching is done.

Using Lemmas~\ref{lem:basic_operation_time},~\ref{lem:ComputeShortCommonSequence},~\ref{lem:ComputePatternRange} and~\ref{lem:pattern_occurrence_lemma1},
we get the following lemma:
\begin{lemma}\label{lem:static_index_lemma}
For a signature encoding $\mathcal{G}$, represented by $\mathcal{H}(f_{\mathcal{A}}, f'_{\mathcal{A}})$,
of size $w$ which generates a text $T$ of length $N$,
there exists a data structure of size $O(w)$ that computes, given a string $P$,
$\mathit{pOcc}_{\mathcal{G}}(P)$ in $O(|P| f_{\mathcal{A}} + \log w \log |P| \log^* M (\log N + \log |P| \log^* M) + q_{w} |\mathit{pOcc}_{\mathcal{S}}(P)|)$ time.
\end{lemma}
\begin{proof}
% If $|\pow{0}{P}| = 1$, $\mathit{pOcc}_{\mathcal{G}}(P) = \mathit{pOcc}_{\mathcal{G}}(P, 1)$ by Lemma~\ref{lem:pattern_occurrence_lemma1}.
% Hence $\mathit{pOcc}_{\mathcal{G}}(P, 1)$ can be computed by a single range reporting query.
% $e \rightarrow \hat{e}^{d}$ with $\hat{e} \rightarrow P[1]$ and $d \geq |P|$.
We focus on the case $|\pow{0}{P}| > 1$ as the other case is easier to be solved.
We first compute the common sequence of $P$ in $O(|P|f_{\mathcal{A}})$ time.
Taking $\mathcal{P}$ in Lemma~\ref{lem:pattern_occurrence_lemma1},
we recall that $|\mathcal{P}| = O(\log |P| \log^* M)$ by Lemma~\ref{lem:common_sequence2}.
Then, in light of Lemma~\ref{lem:pattern_occurrence_lemma1}, $\mathit{pOcc}_{\mathcal{G}}(P)$ can be obtained 
by $|\mathcal{P}| = O(\log |P| \log^* M)$ range reporting queries.
For each query, we spend $O(\log w (\log N + \log |P| \log^* M))$ time to compute $x_1^{(P,j)}, x_2^{(P,j)}, y_1^{(P,j)}$ and $y_2^{(P,j)}$ by Lemma~\ref{lem:ComputePatternRange}.
Hence, the total time complexity is $O(|P| f_{\mathcal{A}} + \log |P| \log^* M ( \log w (\log N + \log |P| \log^* M) + \hat{q}_{w}) + q_{w} |\mathit{pOcc}_{\mathcal{S}}(P)|)
= O(|P| f_{\mathcal{A}} + \log w \log |P| \log^* M (\log N + \log |P| \log^* M) + q_{w} |\mathit{pOcc}_{\mathcal{S}}(P)|)$.
\qed
\end{proof}


\subsection{Dynamic Index for Signature Encoding}\label{subsec:DynIndexSigEnc}
In order to dynamize our static index in the previous subsection,
we consider a data structure for ``dynamic'' two-dimensional orthogonal range reporting
that can support the following update operations:
\begin{itemize}
% \item $\mathit{insert}_{\mathcal{R}}(p, x_{\mathit{succ}}, y_{\mathit{succ}})$:
% Assume that $\mathcal{X} \cup \{ x \}$ and $\mathcal{Y} \cup \{ y \}$ are well defined for a givne point $p = (x, y)$,
% and $x_{\mathit{succ}} = \min \{ x' \in \mathcal{X} \cup \{ \infty_{\mathcal{X}} \} \mid x \leq x' \}$
% and $y_{\mathit{succ}} = \min \{ y' \in \mathcal{Y} \cup \{ \infty_{\mathcal{Y}} \} \mid y \leq y' \}$,
% where $\infty_{\mathcal{X}}$ (resp. $\infty_{\mathcal{Y}}$) represents the largest 
% given a point $p = (x, y)$ such that the ordered sets $\mathcal{X} \cup \{ x \}$ and $\mathcal{Y} \cup \{ y \}$ are well defined,
% $x_{\mathit{pred}} = \max \{ x' \in \mathcal{X} \cup \{ \infty\} \mid x' \leq x \}$ and $x_{\mathit{pred}} = \max \{ x' \in \mathcal{X} \cup \{ \infty\} \mid x' \leq x \}$
% insert $p$ to $\mathcal{R}$ and update $\mathcal{X}$ and $\mathcal{Y}$ accordingly.
\item $\mathit{insert}_{\mathcal{R}}(p, x_{\mathit{pred}}, y_{\mathit{pred}})$:
given a point $p = (x, y)$,
$x_{\mathit{pred}} = \max \{ x' \in \mathcal{X} \mid x' \leq x \}$ and
$y_{\mathit{pred}} = \max \{ y' \in \mathcal{Y} \mid y' \leq y \}$,
insert $p$ to $\mathcal{R}$ and update $\mathcal{X}$ and $\mathcal{Y}$ accordingly.
\item $\mathit{delete}_{\mathcal{R}}(p)$: given a point 
$p = (x,y) \in \mathcal{R}$, delete $p$ from $\mathcal{R}$ and update $\mathcal{X}$ and $\mathcal{Y}$ accordingly.
\end{itemize}
We use the following data structure:
\begin{lemma}[\cite{DBLP:conf/soda/Blelloch08}]\label{lem:RangeQuery}
There exists a data structure
that supports $\mathit{report}_{\mathcal{R}}(x_1,x_2,y_1,y_2)$ 
in $O(\log |\mathcal{R}| + \mathit{occ}(\log |\mathcal{R}| / \log \log |\mathcal{R}|))$ time, 
and $\mathit{insert}_{\mathcal{R}}(p,i,j)$, 
$\mathit{delete}_{\mathcal{R}}(p)$ in amortized $O(\log |\mathcal{R}|)$ time, 
where $\mathit{occ}$ is the number of the elements to output. 
This structure uses $O(|\mathcal{R}|)$ space.~\footnote{
	The original problem considers a real plane in the paper~\cite{DBLP:conf/soda/Blelloch08}, however, 
	his solution only need to compare any two elements in $\mathcal{R}$ in constant time. 
	Hence his solution can apply to our range reporting problem by maintains $\mathcal{X}$ and $\mathcal{Y}$ 
	using the data structure of order maintenance problem proposed 
	by Dietz and Sleator~\cite{DBLP:conf/stoc/DietzS87}, which enables us to 
	compare any two elements in a list $L$ and insert/delete an element to/from $L$ in constant time.
}
\end{lemma}

Now we are ready to prove Theorem~\ref{theo:dynamic_index}.
\begin{proof}[Proof of Theorem~\ref{theo:dynamic_index}]
Our index consists of $\mathcal{H}(f_{\mathcal{A}}, f'_{\mathcal{A}})$ and a dynamic range reporting data structure $\Lambda$ of Lemma~\ref{lem:RangeQuery}
whose $\mathcal{R}$ is maintained as they are defined in the static version.
We maintain $\mathcal{X}$ and $\mathcal{Y}$ in two ways;
self-balancing binary search trees for binary search,
and Dietz and Sleator's data structures for order maintenance.
Then, primary occurrences of $P$ can be computed as described in Lemma~\ref{lem:static_index_lemma}.
Adding the $O(\mathit{occ} \log N)$ term for computing all pattern occurrences from primary occurrences,
we get the time complexity for pattern matching in the statement.
Concerning the update of our index, 
we described how to update $\mathcal{H}$ after $\mathit{INSERT}$ and $\mathit{DELETE}$ in Lemma~\ref{lem:INSERT_DELETE}.
What remains is to show how to update $\Lambda$ when a signature is inserted into or deleted from $\mathcal{V}$.
When a signature $e$ is deleted from $\mathcal{V}$, 
we first locate $e.{\rm left}^R$ on $\mathcal{X}$ and $e.{\rm right}$ on $\mathcal{Y}$,
and then execute $\mathit{delete}_{\mathcal{R}}(e.{\rm left}^R, e.{\rm right})$.
When a signature $e$ is inserted into $\mathcal{V}$, 
we first locate
$x_{\mathit{pred}} = \max \{ x' \in \mathcal{X} \mid x' \leq e.{\rm left}^R \}$ on $\mathcal{X}$ and
$y_{\mathit{pred}} = \max \{ y' \in \mathcal{Y} \mid y' \leq e.{\rm right} \}$ on $\mathcal{Y}$,
and then execute $\mathit{insert}_{\mathcal{R}}((e.{\rm left}^R, e.{\rm right}), x_{\mathit{pred}}, y_{\mathit{pred}})$.
The locating can be done by binary search on $\mathcal{X}$ and $\mathcal{Y}$
in $O(\log w \log N \log^* M)$ time as Lemma~\ref{lem:ComputePatternRange}.
In a single $\mathit{INSERT}(i,Y)$ or $\mathit{DELETE}(i,y)$ operation, 
$O(y + \log N \log^* M)$ signatures are inserted into or deleted from $\mathcal{V}$, where $|Y| = y$.
Hence we get Theorem~\ref{theo:dynamic_index}.
\qed
\end{proof}

